Optimal Resource Procurement and the Price of Causality

This paper studies the problem of procuring diverse resources in a forward market to cover a set $\bf{E}$ of uncertain demand signals $\bf{e}$. We consider two scenarios: (a) $\bf{e}$ is revealed all at once by an oracle (b) $\bf{e}$ reveals itself causally. Each scenario induces an optimal procurement cost. The ratio between these two costs is defined as the {\em price of causality}. It captures the additional cost of not knowing the future values of the uncertain demand signal. We consider two application contexts: procuring energy reserves from a forward capacity market, and purchasing virtual machine instances from a cloud service. An upper bound on the price of causality is obtained, and the exact price of causality is computed for some special cases. The algorithmic basis for all these computations is set containment linear programming. A mechanism is proposed to allocate the procurement cost to consumers who in aggregate produce the demand signal. We show that the proposed cost allocation is fair, budget-balanced, and respects the cost-causation principle. The results are validated through numerical simulations.

==> Counterexample.tex <==
\section{Motivating Examples}
Causality {\em does} have a cost. In this section, we construct two examples to show that $\text{PoC}>1$ is possible.

\subsection{Procure Reserves in Electricity Market}
Uncertainties from demands and renewables create power imbalances in real-time electricity market. The first example considers a system operator who procures energy reserves from a forward capacity market to cover the imbalance signals. Diverse resources are available in the forward capacity market, such as batteries, generators, aggregation of thermostatically controlled loads \cite{hao2015aggregate}, \cite{zhao2017geometric}, among others. The energy output of each resource is bounded and subject to linear constraints, i.e., maximum charging/discharging rates of batteries, ramping constraints for generators, etc. Therefore, the output sequence is constrained in a polytope. 


As an example, consider two batteries that cover an imbalance signal in three periods. The signal is contained in a set $E$, defined as the convex hull of $(0,0,0)$, $(1,1,-2)$ and $(1,1,4)$.  Each unit battery $i$ has a price $p_i$. Let $p_1=3$ and $p_2=1$. In addition, each battery $i$ has a capacity constraint $C_i$ and a maximum charging/discharging rate $r_i$. Let   $C_1=C_2=3$, $r_1=3$ and $r_2=1$. Assume all batteries are empty at time $0$, then the feasible energy output of the first battery satisfies the following linear constraints:
\begin{align}
\label{constraint4battery1}
\begin{cases}
0\leq s_1^1\leq 3; \\
0\leq s_1^1+s_1^2 \leq 3; \\
0\leq s_1^1+s_1^2+s_1^3 \leq 3, \\
-3\leq s_1^t\leq 3, \quad \forall t=1,2,3.
\end{cases}
\end{align}
The feasible energy output of the second battery is as follows:
\begin{align}
\label{constraint4battery2}
\begin{cases}
0\leq s_2^1\leq 3; \\
0\leq s_2^1+s_2^2 \leq 3; \\
0\leq s_2^1+s_2^2+s_2^3 \leq 3, \\
-1\leq s_2^t\leq 1, \quad \forall t=1,2,3.
\end{cases}
\end{align}
According to (\ref{constraint4battery1}) and (\ref{constraint4battery2}), the set of feasible output $S_i$ is a bounded polytope, and clearly, $0\in S_i$.
In this example, the resource procurement problem without causal constraint can be formulated as:
\begin{equation}
\label{resourceprocurementexmaple}
\hspace{-1cm} \min_{\alpha_1,\alpha_2} 3\alpha_1+\alpha_2
\end{equation}
%\quad \quad \quad \quad \quad subject to: 
\begin{subnumcases}{\label{constraint4non_causalexample}}
E \subseteq \alpha_1 S_1 \oplus \alpha_2 S_2  \label{polytopecontainexample} \\
\alpha_1\geq 0,  \alpha_2\geq 0,
\end{subnumcases}
where $E$ is the convex hull of $(0,0,0)$, $(1,1,-2)$, and $(1,1,4)$,  and $S_1$ and $S_2$ are defined by (\ref{constraint4battery1}) and (\ref{constraint4battery2}), respectively. :
\begin{proposition}
\label{solutiontoexample}
The polytope containment problem (\ref{resourceprocurementexmaple}) has a unique solution  $\alpha_1^*=\alpha_2^*=1$.
\end{proposition}
\begin{proof}
The idea is as follows. We first show that $J^*\geq 4$, and $\alpha_1=\alpha_2=1$ is the only possible solution that attains $J^*=4$. Second, we show that $\alpha_1=\alpha_2=1$ satisfies the polytope containment constraint (\ref{polytopecontainexample}). 

To cover $(1,1,4)$, the total maximum rate $\alpha_1 r_1+\alpha_2 r_2$ is at least 4 (otherwise covering $e^3$ is not possible). Therefore, a necessary condition is:
\begin{equation}
\label{condition1}
3\alpha_1 +\alpha_2 \geq 4.
\end{equation}
In addition, to cover $(1,1,4)$, the total capacity $\alpha_1C_1+\alpha_2C_2$ is at least $1+1+4$. Therefore, another necessary condition is:
\begin{equation}
\label{condition2}
3\alpha_1 +3\alpha_2 \geq 6.
\end{equation}
Combining (\ref{condition1}) and (\ref{condition2}), the optimal value to the following problem is an upper bound for $J^*$:
\begin{equation}
\label{upperbound4example}
\hspace{-0cm} \min_{\alpha_1,\alpha_2} 3\alpha_1+\alpha_2
\end{equation}
%\quad \quad \quad \quad \quad subject to: 
\begin{subnumcases}{\label{constraint4upperbound}}
3\alpha_1 +\alpha_2 \geq 4,   \\
3\alpha_1 +3\alpha_2 \geq 6.
\end{subnumcases}
The optimal value of (\ref{upperbound4example}) is $4$, and the unique solution is $\alpha_1=\alpha_2=1$. Therefore, $\alpha_1=\alpha_2=1$ is necessary. 

Next we show that $\alpha_1=\alpha_2=1$ is sufficient, i.e., the polytope containment constraint (\ref{polytopecontainexample}) is satisfied.  To see this, note that both $E$ and $S_1\oplus S_2$ are convex. Therefore, (\ref{polytopecontainexample}) is equivalent to the vertices of $E$ contained in $S_1 \oplus S_2$. This trivially holds for the vertex $(0,0,0)$ and the vertex $(1,1,-2)\in S_1$. The other vertex $(1,1,4)$ can be decomposed into $(0,0,3)\in S_1$ and $(1,1,1)\in S_2$. This completes the proof.
\end{proof}

To show that $\text{PoC}>1$, it suffices to prove  the operator can not find any causal policy to cover all signals in $E$ when $\alpha_1=\alpha_2=1$. We summarize it as follows: 
\begin{proposition}
\label{counterexample}
Assume $\alpha_1=\alpha_2=1$, then given any causal policy $\gamma(\cdot)$, at least one of the imbalance signals $(1,1,-2)$, $(1,1,4)$ can not be covered by $\gamma(\cdot)$. 
\end{proposition}
\begin{proof}
The first two elements of $(1,1,-2)$ and $(1,1,4)$ are the same. Since $\gamma(\cdot)$ is causal, the allocation for the first two periods should also be the same for $(1,1,-2)$ and $(1,1,4)$.  To cover the signal $(1,1,4)$, the unique allocation is to exclusively use the second battery for the first two periods, and then use both batteries at the third period, i.e., $\gamma_1^1(\cdot)=\gamma_1^2(\cdot)=0$, $\gamma_1^3(\cdot)=3$, and $\gamma_2^1(\cdot)=\gamma_2^2(\cdot)=\gamma_2^3(\cdot)=1$.  On the other hand, if we exclusively use the second battery for the first two periods, then $(1,1,-2)$ cannot be covered, since at time $3$, the maximum discharging rate of the second battery is $1<2$. This completes the proof. 
\end{proof}









\subsection{Procure Virtual Machines from a Cloud Provider}
Consider a company that procures virtual machine {\em instances} from a cloud provider (such as Amazon EC2) to serve the workloads from users. It has two types of workloads: (a) transactional workloads, (b) non-interactive batch workloads.  Transactional workloads such as web applications are highly unpredictable and require immediate response. On the other hand,  non-interactive batch workloads can be predicted and only require completion within a specified time frame \cite{garg2011sla}. For example, a financial institution uses transactional workloads to trade stocks and query indices, and uses non-interactive workloads to analyze investment portfolio and model stock performance \cite{carrera2008enabling}. 

The company purchases {\em on-demand instances} from cloud providers to serve these workloads. On-demand instances can be requested at any time. It is charged in a pay-as-you-go manner with a specified {\em price per unit time}. For instance, Amazon ECS adopts a price-per-hour policy that rounds up partial hours of usage \cite{amazonec2}. Note that new instances cannot be initialized instantaneously. Typically, there is a delay of several minutes \cite{li2010cloudcmp} due to hardware resource allocation and the boot of new systems. Therefore, the company should procure enough instances in advance, instead of reactively purchasing instances after the workload arrives. This motivates the following problem: how many instances are enough to serve all workloads over some horizon(e.g., 20 minutes)?

To tackle this problem, we model the instances,  non-interactive workloads  and transactional workloads as follows:

\subsubsection{Instances}
Without loss of generality, we assume all instances are homogeneous, and the length of each period is $1$. We model an instance as a unit resource. The output of the resource is $s_1^t$, which represents the fraction of time the instance works during the period $t$. Accordingly, $s_1^t$ satisfies the following constraint:
\begin{equation}
\label{feasibleinstance}
0\leq s_1^t \leq 1, \quad \forall t\in \mathcal{T},
\end{equation}
where $\mathcal{T}=\{1,\ldots,T\}$. Let $s_1=(s_1^1,\ldots,s_1^T)$, and define $S_1=\{s_1|0\leq s_1^t \leq 1, \forall t\in \mathcal{T}\}$.  Clearly, $S_1$ is a hyper-box.  


\subsubsection{Non-Interactive Batch Workloads}
We model the collection of non-interactive workloads as a non-scalable resource.  In particular, consider $M$ non-interactive workloads. Each of them has an arrival time $a_m$, a deadline $d_m$ and a computation time $c_m$, such that $c_m\leq d_m-a_m$. Assume the workloads can be interrupted, and  each workload can be assigned to at most one instance at a time. Let $r_m^t$ denote the fraction of instance computation time allocated to workload $m$ over the period $t$, then we have $0\leq r_m^t \leq 1$.  Denote $s_2^t$ as the total fraction of instance computing time {\em provided} by all batch workloads. Since the workloads {\em demand} computing resources, $s_2^t$ is negative, and satisfies the following constraints:
\begin{subnumcases}{\label{constraintofS4CC}}
s_2^t=-\sum_{m=1}^M r_m^t, \quad \forall t\in \mathcal{T} \label{negativeconst} \\
\sum_{t=1}^T r_m^t =c_m,  \quad \forall m\in \mathcal{M}, \label{negativeconst2}\\
0\leq r_m^t\leq 1,  \quad\forall a_m\leq t \leq d_m, \\
r_m^t=0,  \quad \quad \forall t<a_m, \quad \forall t>d_m. \label{negativeconst4}
\end{subnumcases}
where $\mathcal{M}=\{1,\ldots,M\}$, and (\ref{negativeconst2})-(\ref{negativeconst4}) ensures all workloads to be completed by the deadline. Let $s_2=(s_2^1,\ldots,s_2^T)$, and define $S_2$ as the set of $s_2$ that satisfies (\ref{constraintofS4CC}). It can be verified that $S_2$ is a bounded and convex polytope. 








\subsubsection{Transactional Workloads}
We model transactional workloads as a sequence of random signals. At time $t$, all transactional workloads together require $e^t$ amount of instance computation time. Let $e=(e^1,\ldots,e^T)$. Assume that $e$ only takes value in a polytope  $E \subset \mathbb{R}^T$. In this case, both $S_1$, $S_2$ and $E$ are polytopes. Assumption \ref{asusmptiononpolytope} and Assumption \ref{asusmptiononresource} are satisfied. 



As an example, consider  $E$ as the convex hull of $(0,0,0,0)$, $(1,0.5,1.5,2)$, and $(1,2,1,1)$.  Assume there are two non-interative workloads with $a_1=1$, $d_1=2$, $c_1=1$ and $a_2=1$, $d_2=4$, $c_2=2$. In this case, it can be verified that (\ref{constraintofS4CC}) is equivalent to:
\begin{align}
\label{exampleofccnonscale}
\begin{cases}
\sum_{t=1}^4 s_2^t=-3, \\
-2\leq s_2^t\leq 0, \quad \forall t=1,2, \\
-1\leq s_2^t\leq 0, \quad \forall t=3,4. 
\end{cases}
\end{align}
The resource procurement problem without causality constraint is as follows:
\begin{equation}
\label{resourceprocurementexmaplecc}
\hspace{-1cm} \min_{\alpha_1} \alpha_1
\end{equation}
%\quad \quad \quad \quad \quad subject to: 
\begin{subnumcases}{\label{constraint4non_causalexamplecc}}
E \subseteq \alpha_1 S_1 \oplus S_2  \label{polytopecontainexamplecc} \\
\alpha_1\geq 0.
\end{subnumcases}
where $E$ is the convex hull of $(0,0,0,0)$, $(1,0.5,1.5,2)$, and $(1,2,1,1)$,  and $S_1$ and $S_2$ are defined as (\ref{feasibleinstance}) and (\ref{exampleofccnonscale}), respectively. 
\begin{proposition}
\label{solutiontoexamplecc}
The polytope containment problem (\ref{resourceprocurementexmaplecc}) has a unique solution  $\alpha_1^*=2$.
\end{proposition}
The proof of Proposition \ref{solutiontoexamplecc} is omitted, since it is similar to that of Proposition \ref{solutiontoexample}. 
To show that $PoC>1$, it suffices to prove there is no causal policy to cover all signals in $E$ when $\alpha_1^*=2$. 
\begin{proposition}
\label{coundertoexamplecc}
Assume $\alpha_1=2$, then given any causal policy $\gamma(\cdot)$, at least one of the signals $(1,2,1,1)$, $(1,0.5,1.5,2)$ can not be covered by $\gamma(\cdot)$.
\end{proposition}
\begin{proof}
Since $\alpha_1=2$, two instances are available. At each time, the instances have to be allocated to transactional workloads (random signals) first, since they require immediate response. Consider the two signals $(1,2,1,1)$ and $(1,0.5,1.5,2)$. After the  instances are allocated to them, the remaining instances are $(1,0,1,1)$ and $(1,1.5,0.5,0)$, respectively.  
In the former case $(1,0,1,1)$, the unique feasible schedule for non-interactive batch workloads is $r_1^1=1$, $r_1^2=0$, and $r_2^1=0$, $r_2^2=0$, $r_2^3=1$, $r_2^4=1$. Since the two signals are the same at time 1, due to causality, the schedules should be  the same at time one. This dictates that for the case $(1,1.5,0.5,0)$, $r_1^1=1$ and $r_2^1=0$. However, the second batch workload cannot be finished by the deadline. This is because the maximum values of $r_2^2$, $r_2^3$ and $r_2^4$ are $1$,  $0.5$ and $0$, respectively. This indicates $r_2^1+r_2^2+r_2^3+r_2^4<2$. This completes the proof.
\end{proof}


==> Exactpoc.tex <==
\section{Some Special Cases}
This section computes the price of causality for some special cases. We first construct a few examples to identify the key factors that contribute to $PoC>1$. Then, we focus on a battery example and obtain the exact price of causality. 


\subsection{Key Factors for $PoC>1$}
Consider the following three cases:  


\subsubsection{Resources in a Hyper-Rectangle}
First, assume that $S_i$ is a hyper-rectangle: $S_i=\{s_i\in \mathbb{R}^T |
\underline{s}_i^t \leq s_i^t  \leq \bar{s}_i^t, t\in \mathcal{T} \}$. Under  Assumption \ref{asusmptiononpolytope} and Assumption  \ref{asusmptiononresource},  the price of causality is 1:
\begin{proposition}
\label{poais1_2}
For $\forall i\in \mathcal{N}$, let $S_i$ be a hyper-rectangle: $S_i=\{s_i\in \mathbb{R}^T |
\underline{s}_i^t \leq s_i^t  \leq \bar{s}_i^t, t\in \mathcal{T} \}$.  Under Assumption \ref{asusmptiononpolytope} and Assumption \ref{asusmptiononresource}, we have $\text{PoC}=1$.
\end{proposition}
\begin{proof}
Let $\alpha^*=(\alpha_1^*,\ldots,\alpha_N^*)$ be the optimal solution to the resource procurement problem (\ref{resourceprocurement}). It suffices to construct a causal policy that covers all $e\in E$ under $\alpha^*$. To this end, define $\big(\gamma_1^t(e^{1:t}), \ldots, \gamma_N^t(e^{1:t})\big) $ as any  vector that:
\begin{align*}
\begin{cases}
e^t=\sum_{i=1}^N \gamma_i^t(e^{1:t}), \quad \forall t\in \mathcal{T}, \\
\alpha_i^*\underline{s}_i^t\leq \gamma_i^t(e^{1:t})  \leq \alpha_i^*\bar{s}_i^t, \quad \forall i\in \mathcal{N}, t\in \mathcal{T}.
\end{cases}
\end{align*}
The above allocation policy is causal, and it exists. If it does not exist,  then it indicates that there is some $t$ such that $e^t<\sum_{i=1}^N \alpha_i^*\underline{s}_i^t$ or $e^t>\sum_{i=1}^N \alpha_i^*\bar{s}_i^t$. This contradicts  (\ref{polytopecontain}).  For the same reason, it covers all $e\in E$. This completes the proof.
\end{proof}


\subsubsection{Identical Resources}
Second, assume that resources are identical up to a scale factor. In this case, the price of causality is also 1:
\begin{proposition}
\label{poais1_3}
Assume there exists a $\delta_i\in \mathbb{R}$, such that $\delta_iS_i=\delta_jS_j$ for  $\forall i,j\in \mathcal{N}$.    Under Assumption \ref{asusmptiononpolytope} and Assumption  \ref{asusmptiononresource}, we have $\text{PoC}=1$.
\end{proposition}
\begin{proof}
Let $S=\delta_iS_i$. The polytope containment constraint (\ref{polytopecontain}) becomes:
\begin{equation}
\label{identialrourceproofinter}
E\subseteq \dfrac{\alpha_1}{\delta_1}S \oplus \cdots \oplus \dfrac{\alpha_N}{\delta_N}S.  
\end{equation}
Let $\sigma_i=\alpha_i/\delta_i$, then (\ref{identialrourceproofinter}) is equivalent to:
\begin{equation}
\label{identialproofimport}
E\subseteq  \sum_{i=1}^N \sigma_i S.
\end{equation}
Consider the following allocation policy:
\begin{equation}
\label{allocationpolicyidential}
\gamma_i^t(e^{1:t})=\dfrac{\sigma_i}{\sum_{i=1}^N \sigma_i} e^t.
\end{equation}
Clearly, (\ref{allocationpolicyidential}) is causal. To prove it covers all $e\in E$, we note that (\ref{identialproofimport}) is the same as $\dfrac{\sigma_i}{\sum_{i=1}^N \sigma_i} E \subseteq \sigma_i S$. Therefore:
\begin{equation*}
\dfrac{\sigma_i}{\sum_{i=1}^N \sigma_i}  e \in \sigma_i S=\alpha_i S_i, \quad \forall e\in E.
\end{equation*}
This completes the proof.
\end{proof}


\subsubsection{Signals in a Hyper-Rectangle}
Third, consider $E$ as a hyper-rectangle: $E=\{e\in \mathbb{R}^T |
\underline{e}^t \leq e^t  \leq \bar{e}^t, \forall t\in \mathcal{T} \}$. Under Assumption \ref{asusmptiononresource},  the price of causality could be greater than 1:
\begin{proposition}
\label{poais1}
Assume that $E$ is a hyper-rectangle $E=\{e\in \mathbb{R}^T |
\underline{e}^t \leq e^t  \leq \bar{e}^t, \forall t\in \mathcal{T}\}$, and $S_i$ satisfies Assumption~ \ref{asusmptiononresource},  then it is possible that  $\text{PoC}>1$.
\end{proposition}
\begin{proof}
It suffices to construct an example with $PoC>1$. Consider to use two batteries to cover signals in $E=\{e|0\leq e^1 \leq 1, 0\leq e^2 \leq 1, -5 \leq e^3 \leq 7 \}$. The capacity of each battery is $C_1=9$ and $C_2=5$, and the maximum charging/discharging rate is  $r_1=2$, $r_2=5$. At time $0$, the initial state of charge is $33\%$ and $40\%$, respectively. Let $p_1=2$ and $p_2=5$. In this case, we can show that the optimal solution to (\ref{resourceprocurement}) is $\alpha_1=\alpha_2=1$. However, we can also show that when $\alpha_1=\alpha_2=1$, no causal policy can be found to cover both $(0,0,-5)$ and $(0,0,7)$. The proof is similar to that in Section III-A, and is therefore omitted.
\end{proof}

\begin{remark}
According to Proposition \ref{poais1_2}-\ref{poais1}, the  main cause for $PoC>1$ is the dynamics and the diversity  of the resources.  The price of causality is greater than 1 only if both factors are observed. Surprisingly, the dynamics of the signals are irrelevant.
\end{remark}









\subsection{Exact Price of Causality for Batteries}
Consider the resource to be a group of batteries. For simplicity, assume that all batteries are scalable resource.  Each battery $i$ has a capacity constraint $C_i$ and a maximum charging/discharging rate $r_i$. 
Denote the initial state of charge for the $i$th battery (in percentage value) as $\theta_i$, then  $S_i$ contains all $s_i\in \mathbb{R}^T$ that satisfy the following constraints:
\begin{numcases}{}
-r_i\leq s_i^t \leq r_i, \quad \forall t\in \mathcal{T},  \label{rateconstraint}\\
0\leq \theta_iC_i+\sum_{k=1}^t s_i^k\leq C_i, \quad \forall t\in \mathcal{T}, i\in \mathcal{N}, \label{capacityconstaint}
\end{numcases}
where (\ref{rateconstraint}) is the charging/discharging rate constraint, and (\ref{capacityconstaint}) is the capacity constraint. 


Assume $E$ is the Minkowski sum of $S_i$, i.e., $E=S_1\oplus S_2 \oplus \cdots \oplus S_N$. We  show that $J^{**}$ can be obtained by solving a linear program. 
\begin{theorem}
\label{proposition4exactpoa}
Consider a group of batteries. Assume  their parameters satisfy $\sum_{i=1}^N C_i\leq 2\sum_{i=1}^N r_i $, then there exists $T_0>0$, so that for $\forall T> T_0$, as long as $E=S_1\oplus S_2 \oplus \cdots \oplus S_N$,  $J^{**}$ is the optimal value for the following linear program:
\begin{equation}
\label{poaaslinearprogramming}
\hspace{-2cm} \min_{\alpha_1,\ldots,\alpha_N} \sum_{i=1}^{N} \alpha_i p_i
\end{equation}
%\quad \quad \quad \quad \quad subject to: 
\begin{subnumcases}{\label{constraint4poaaslinearprogramming}}
\sum_{i=1}^N \alpha_i r_i \geq \sum_{i=1}^N r_i, \label{constraint1forpoaaslp}\\
\sum_{i=1}^{N} \alpha_i  \min (2r_i,C_i)\geq\sum_{i=1}^N C_i, 
 \label{constraint2forpoaaslp}
\end{subnumcases}
 where $\min (a,b)$ is the lesser of $a$ and $b$.
\end{theorem}
To prove Theorem \ref{proposition4exactpoa}, we need the following lemma:
\begin{lemma}
\label{lemmaforbigtheor}
Under the assumptions of Theorem \ref{proposition4exactpoa}, there exist $T_0$ such that for all $T> T_0$,  there exists $(e^1,\ldots,e^{T-1})$ that satisfies $(e^1,\ldots,e^{T-1},\sum_i C_i/2) \in E$ and $(e^1,\ldots,e^{T-1},-\sum_i C_i/2) \in E$. 
\end{lemma}
\begin{proof}
since $E=S_1\oplus S_2 \oplus \cdots \oplus S_N$,  it suffices to construct a sequence $(e^1,\ldots, e^{T-1})$ and two allocation policies  to cover $(e^1,\ldots,e^{T-1},\sum_i C_i/2)$ and $(e^1,\ldots,e^{T-1},-\sum_i C_i/2)$ using unit batteries.
Without loss of generality,  assume that all batteries are empty at time $0$, i.e., $\theta_i=0$. If $\theta_i>0$, we can construct a sequence of signals to empty all batteries first and then concatenate this sequence with $(e^1,\ldots,e^{T-1})$. 


Consider the first allocation policy to satisfy the following: 
\begin{itemize}
\item  Each battery $i$ is charged by no more than $r_i$ for all $t \leq T-1$, i.e.,  $\sum_{k=1}^t s_i^k\leq r^i$, $\forall t\leq T-1$,
\item The ($i+1$)th battery is used only if the $i$th battery is already charged by $r_i$, i.e., $s_i^t>0$ only if $s_j^t=r_j$ for all $j<i$.
\end{itemize}
Under this policy, the maximum total power the batteries can provide at time $t$ is $\sum_{i=1}^{N} r_i- \sum_{k=1}^{t-1} e^k$. On the other hand, consider a signal sequence  $(e^1,\ldots,e^{T-1})$  that satisfies:
\begin{align}
\label{constructsequence}
\begin{cases}
 \sum_{t=1}^{T-1} e^t=\dfrac{1}{2}\sum_{i=1}^N C_i, \\
 e^t\geq 0,  \quad \forall 0\leq t \leq T-1.
 \end{cases}
\end{align}
Clearly, for any $t\leq T-1$, as long as  $(e^1,\ldots,e^{T-1})$  satisfies (\ref{constructsequence}), we have
$e^t\leq \sum_{i=1}^N C_i/2-\sum_{k=1}^{t-1} e^k$. Since $\sum_{i=1}^{N} r_i\geq \sum_{i=1}^N C_i/2$, we have:
\begin{equation*}
e^t\leq \sum_{i=1}^N C_i/2-\sum_{k=1}^{t-1} e^k \leq \sum_{i=1}^{N} r_i- \sum_{k=1}^{t-1} e^k.
\end{equation*}
Therefore, the first policy covers all  $(e^1,\ldots,e^{T-1})$ that satisfies (\ref{constructsequence}). In addition, since each battery $i$ are charged by at most $r_i$ at the first $T-1$ steps, all batteries can be discharged to empty at time $T$. Therefore, it is able to cover $-\sum_{i=1}^N C_i/2$ at time $T$. 



The second policy satisfies the following conditions: 
\begin{itemize}
\item  Each battery $i$ is charged by no more than $C_i-r_i$ for all $t \leq T-1$. Formally, $\sum_{k=1}^t s_i^k\leq C_i-r^i$, $\forall t\leq T-1$,
\item The ($i+1$)th battery is used only if the $i$th battery is already charged by $C_i-r_i$, i.e., $s_i^t>0$ only if $s_j^t=C_j-r_j$ for all $j<i$.
\end{itemize}
Trivially, under this policy, we can find a $T_0>0$ so that $(e^1,\ldots,e^{T_0})$ can be covered by the unit batteries and satisfies:
\begin{align*}
\begin{cases}
 \sum_{t=1}^{T_0} e^t=\dfrac{1}{2}\sum_{i=1}^N C_i, \\
 e^t\geq 0,  \quad \forall 0\leq t \leq T_0.
 \end{cases}
\end{align*}
For any $T> T_0$, let $(e^1,\ldots,e^{T-1})=(e^1,\ldots,e^{T_0}, 0,\ldots,0)$. Since $(e^1,\ldots,e^{T_0})$ is covered by unit batteries,  $(e^1,\ldots,e^{T-1})$ is also covered. 
In addition, since each battery $i$ is charged by at most $C_i-r_i$,  the policy  also guarantees to cover $\sum_{i=1}^N C_i/2$ at time $T$. 
This completes the proof of Lemma \ref{lemmaforbigtheor}.
\end{proof}



Using Lemma \ref{lemmaforbigtheor}, the proof of Theorem \ref{proposition4exactpoa} is as follows:





\begin{proof}
It suffices to show that (\ref{constraint4poaaslinearprogramming}) is both necessary and sufficient for  (\ref{constraint4causal_formualtion}). To prove necessity, we first note that (\ref{constraint1forpoaaslp}) is clearly necessary: if (\ref{constraint1forpoaaslp}) is not satisfied, we can construct some signal such that $e^t=\sum_{i=1}^N r_i$ for some $t$, then this signal can not be covered. To show that (\ref{constraint2forpoaaslp}) is also necessary, we note that according to Lemma \ref{lemmaforbigtheor}, there exist $T_0$ and $(e^1,\ldots,e^{T-1})$ such that $(e^1,\ldots,e^{T-1},\sum_i C_i/2) \in E$ and $(e^1,\ldots,e^{T-1},-\sum_i C_i/2) \in E$. Since the first $T-1$ elements of the signals are the same, a causal policy should make the same allocation decision for these two cases in the first $T-1$ steps. Therefore, at time $T$, the batteries should satisfy both $\sum_iC_i/2$ and $-\sum_iC_i/2$. Let $x_i^t$ denote the state of charge of battery $i$ at time $t$, i.e., $x_i^t=\theta_iC_i+\sum_{k=1}^t s_i^t$, then the following conditions should hold:
\begin{numcases}{}
\sum_{i=1}^N \alpha_i \min (r_i,C_i-x_i^{T-1} ) \geq \dfrac{1}{2} \sum_{i=1}^N C_i,  \label{conditions4proof1}\\
\sum_{i=1}^N \alpha_i \min (r_i,x_i^{T-1} ) \geq \dfrac{1}{2} \sum_{i=1}^N C_i. \label{conditions4proof2}
\end{numcases}
where $\min(r_i,C_i-x_i^{T-1})$ is the maximum energy battery $i$ can absorb at time $T$, and $\min(r_i,x_i^{T-1})$ is the maximum energy battery $i$ can provide at time $T$. 	Clearly, (\ref{conditions4proof1}) is necessary for the policy to cover $\sum_{i=1}^N C_i/2$ at time $T$, and (\ref{conditions4proof2}) is necessary for the policy to cover $-\sum_{i=1}^N C_i/2$ at time $T$. Adding up (\ref{conditions4proof1}) and (\ref{conditions4proof2}), and using the following inequality (can be verified by discussing different cases):
\begin{equation}
\min(r_i,C_i-x_i^{T-1})+\min(r_i,x_i^{T-1})\leq \min(2r_i,C_i),
\end{equation}
we obtain
(\ref{constraint2forpoaaslp}) as a necessary condition. Therefore,  (\ref{constraint4poaaslinearprogramming}) is necessary for  (\ref{constraint4causal_formualtion}).


To prove sufficiency, we construct a causal policy that covers all signals in $E$ when (\ref{constraint4poaaslinearprogramming})  holds.  Rank all batteries in a decreasing order of $C_i/r_i$. Without loss of generality, assume battery $1$ has the largest $C_i/r_i$, battery $2$ has the second largest, and so on. Divide $\mathcal{N}$ into three subsets: $\mathcal{N}_1=\{i\in \mathcal{N}|C_i=r_i \}$, $\mathcal{N}_2=\{i\in \mathcal{N}|r_i<C_i<2r_i \}$, and $\mathcal{N}_3=\{i\in \mathcal{N}|C_i\geq 2r_i \}$. 

To enhance readability, we first prove the result for a simple example, then we discuss how to generalize the proof to all other cases. As an example, consider  a group of three batteries with the following parameter: $C_1=r_1$, $C_2\geq 2r_2$, and  $C_3 \geq 2r_3$. We propose a causal allocation policy that divides each battery into a few blocks, and uses each block according to an alternating order to construct a virtual battery. The idea is illustrated in Figure \ref{allocation}, where the first battery contributes one block $\alpha_1 r_1$, the second battery contributes two identical blocks $\alpha_2 r_2$, and the third battery contributes two identical blocks $\alpha_3 r_3$. These blocks are arranged in the following order: $\alpha_3 r_3$, $\alpha_2 r_2$, $\alpha_1 r_1$, $\alpha_3 r_3$, $\alpha_2 r_2$, as illustrated in Figure \ref{allocation}. 
\begin{figure}[t]%
\centering
\includegraphics[width = 0.4\linewidth]{allocation}
\caption{The causal allocation: battery $1$ is one block $\alpha_1r_1$, battery $2$ is divided into 2 identical blocks $\alpha_2 r_2$, and battery $3$ is divided into two identical  blocks $\alpha_3 r_3$. These blocks are arranged in the following order: $\alpha_3r_3$, $\alpha_2r_2$, $\alpha_1r_1$, $\alpha_3r_3$, $\alpha_2r_2$.}
\label{allocation}
\end{figure}
Formally, the allocation in Figure \ref{allocation} can be described as one that respects the following conditions:
\begin{align}
\label{causalpolicy}
\begin{cases}
x_2^t= 0 \text{ unless } x_3^t=\alpha_3r_3, \\
x_1^t=0 \text{ unless } x_2^t\geq \alpha_2r_2  \text{ and } x_3^t\geq \alpha_3 r_3, \\
x_3^t\leq \alpha_3r_3 \text{ unless } x_1^t=\alpha_1C_1, \\
x_2^t\leq \alpha_2r_2 \text{ unless }  x_1^t=\alpha_1C_1 \text{ and }x_3^t=2\alpha_3r_3 , \\
x_2^t\leq 2\alpha_2r_2, \quad x_3^t\leq 2\alpha_3r_3.
\end{cases}
\end{align}
Clearly, this single battery has capacity $\alpha_1C_1+2\alpha_2r_2+2\alpha_2r_3$. Due to (\ref{constraint2forpoaaslp}), it is greater than $\sum_iC_i$. In addition, the charging/discharging rate is $\sum_i\alpha_ir_i$. Due to (\ref{constraint1forpoaaslp}), it is greater than $\sum_ir_i$. Therefore, it covers all signals in $E=S_1\oplus S_2 \oplus S_3$.

Next we generalize the proof idea to all possible cases. Note that in the example, $\mathcal{N}_1=\{1\}$, $\mathcal{N}_2=\emptyset$, and $\mathcal{N}_3=\{2,3\}$. We simply need to generalize the result to all possible combinations of $\mathcal{N}_1$, $\mathcal{N}_2$ and $\mathcal{N}_3$. First, we note that if there are more than one battery in $\mathcal{N}_1$, there is no difference, as these batteries can be used as a single one. Second, if there are more than two batteries in $\mathcal{N}_3$, then the proof idea of the example simply goes through. Third, if $\mathcal{N}_2$ is non-empty, i.e., $j\in \mathcal{N}_2$, then we remove battery $j$ from $\mathcal{N}$, divide it into two batteries, and then place these two batteries back to $\mathcal{N}$. In particular, denote these two new batteries as $i=N+1$ and $i=N+2$, such that $\alpha_{N+1}=\alpha_{N+2}=\alpha_j$, $C_{N+1}=r_{N+1}=2r_i-C_i$ and $C_{N+2}=2C_i-2r_i$, $r_{N+2}=C_i-r_i$. Note that $C_{N+1}+C_{N+2}=C_{j}$ and $r_{N+1}+r_{N+2}=r_j$. Therefore, it is a division of battery $j$.  
After this operation, we have $N+1\in \mathcal{N}_1$ and $N+2\in \mathcal{N}_3$.  Apply this operation for all  $i\in \mathcal{N}_2$ until $\mathcal{N}_2=\emptyset$, then we are back to the case of the example. This completes the proof.
\end{proof}
Under the assumption of Theorem \ref{proposition4exactpoa}, we can solve  (\ref{resourceprocurement_linear}) and (\ref{poaaslinearprogramming}) to derive $J^*$ and $J^{**}$, respectively. This provides the exact price of causality.



\begin{remark}
To allocate $e^t$ according to (\ref{causalpolicy}), the initial state of charge $\theta=(\theta_1,\ldots,\theta_N)$ should also satisfy (\ref{causalpolicy}). This inherently assumes that the operator can  arbitrarily  set $\theta$ after procuring the resources. We can easily incorporate this in the resource procurement problems (\ref{resourceprocurement}) and (\ref{resourceprocurement_causality}) by viewing $S_i$ as a set that depends on $\theta_i$ and including $\theta_i$ as an additional decision variable. We refrain from doing this to simplify notation and enhance readability. It is easy to verify that all results in the paper hold when $\theta_i$ is also a decision variable. 
\end{remark}































\begin{figure*}
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
\includegraphics[width=0.95\textwidth]{figure1} % first figure itself
 \caption{The  procurement costs under different price ratio $\kappa$.}
\label{figure1}               
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
        \centering
\includegraphics[width = 0.85\linewidth]{upperbound}
\caption{$J^{**}$ and upper bound under affine causal policy.}
\label{upperbound} 
    \end{minipage}
\end{figure*}












==> Upperbound.tex <==



\section{Upper Bound on the Price of Causality}
This section focuses on the computation of the price of causality. First, we show that $J^*$ can be solved by linear programming. Second, we obtain an upper bound of $J^{**}$ by restricting the causal policy to be affine. This provides an upper bound on the price of causality.




\subsection{Solving $J^*$ by linear programming}
To tackle the resource procurement problem (\ref{resourceprocurement}), we represent $E$ as the convex hull of a set of vertices. Denote each vertex as $v_i$, then $E=conv(v_1,\ldots,v_K)$. Different from $E$,  we represent $S_i$ as the intersection of half-spaces $S_i=\{s_i\in \mathbb{R}^T| A_is_i\leq B_i\}$. For scalable resources, $\alpha_iS_i=\{s_i\in \mathbb{R}^T| A_is_i\leq \alpha_iB_i\}$ for $\forall i\in \mathcal{N}_s$.
\begin{remark}
The polytopes $E$ and $S_i$ are represented in different ways: $E$ is a convex full of vertices (vertex representation), and $S_i$ is the intersection of  half-spaces (H-representation). These two representations are equivalent, since we can transform from one to another. However, interestingly, the difficulty of solving (\ref{resourceprocurement}) crucially depends on the choice of polytope representations. 
\end{remark}

Since $E$ is convex, the Minkowski sum of $\alpha_iS_i$ is also convex. Therefore, the set containment constraint (\ref{polytopecontain}) is equivalent to all vertices of $E$ contained in the Minkowski sum of $\alpha_iS_i$: 
\begin{equation}
\label{intermediate}
v_k\in \alpha_1 S_1 \oplus \alpha_2 S_2 \oplus \cdots \oplus \alpha_N S_N , \quad \forall  k\in \mathcal{K},
\end{equation}
where $\mathcal{K}=\{1,\ldots,K\}$.
This leads to the following result:
\begin{theorem}
\label{noncausalresourceprocurement}
The resource procurement problem (\ref{resourceprocurement}) is equivalent to:
\begin{equation}
\label{resourceprocurement_linear}
\hspace{-4cm} \min \sum_{i=1}^{N} \alpha_i p_i
\end{equation}
%\quad \quad \quad \quad \quad subject to: 
\begin{subnumcases}{\label{constraint4causalcc}}
v_k=\sum_{i=1}^N q_{i,k}, \quad \forall k\in \mathcal{K}, \label{conservationofall_linearcc}\\
A_iq_{i,k}\leq \alpha_iB_i,  \quad \forall k\in \mathcal{K}, i\in \mathcal{N}, \label{feasibleset_icc}\\
\alpha_i=1, \quad \forall i\in \mathcal{N}\setminus \mathcal{N}_s, \\
\alpha_i\geq 0,  \quad \forall i\in \mathcal{N}.
\end{subnumcases}
The decision variables are $\alpha_1, \ldots, \alpha_N$ and $q_{i,k}\in \mathbb{R}^T$, $\forall i,k$.
\end{theorem}
\begin{proof}
Comparing (\ref{resourceprocurement}) with (\ref{resourceprocurement_linear}), it suffices to show that the polytope containment constraint (\ref{polytopecontain}) is equivalent to (\ref{conservationofall_linearcc}) and (\ref{feasibleset_icc}). As $E$ and the Minkowski sum of $\alpha_iS_i$ are both convex, (\ref{polytopecontain}) is equivalent to (\ref{intermediate}).  
Denote $q_{i,k}\in \mathbb{R}^T$ as the allocation of $v_k$ to the $i$th resource, then the constraint (\ref{intermediate}) can be written as follows:
\begin{align}
\label{intermediatecc2}
\begin{cases}
v_k=\sum_{i=1}^N q_{i,k}, \quad \forall k\in \mathcal{K}, \\
q_{i,k}\in \alpha_i S_i, \quad \forall k\in \mathcal{K}, i\in \mathcal{N}. 
\end{cases}
\end{align} 
Clearly, (\ref{intermediatecc2}) is equivalent to (\ref{conservationofall_linearcc}) and (\ref{feasibleset_icc}). This completes the proof.
\end{proof}

Based on Theorem \ref{noncausalresourceprocurement}, $J^*$ can be solved via linear programming. 




















\subsection{Upper bound of $J^{**}$ by linear programming}
When the allocation policy is causal, the resource procurement problem (\ref{resourceprocurement_causality}) is essentially a robust optimization over functions \cite{ben2009robust}. This is a rather challenging problem in general. Here we restrict the causal allocation policy to be affine and obtain an upper bound on $J^{**}$.



\subsubsection{Proportional Allocation Policy}
First, consider a simple causal policy that allocates random signals according to a fixed proportion $\beta=(\beta_1,\ldots,\beta_N)$. Let $\sum_{i=1}^N \beta_i=1$, and define the policy as $\gamma_i^t(e^{1:t})=\beta_i e^t$. We refer to it as the proportional allocation policy. Under this policy, the set $\mathcal{Q}$ becomes:
\begin{equation}
\label{Qforproposition}
\mathcal{Q}=\{e|\beta_i(e)\in \alpha_i S_i, \forall i\in \mathcal{N} \}.
\end{equation}
This indicates the constraint (\ref{polytopecontain_causal}) is equivalent to $\beta_iE\subseteq \alpha_iS_i$ for all $i\in \mathcal{N}$,  and the resource procurement problem (\ref{resourceprocurement_causality}) reduces to the following:
\begin{equation}
\label{causality4proportaional}
\hspace{-1cm} \min_{\alpha_1,\ldots,\alpha_N, \beta} \sum_{i=1}^{N} \alpha_i p_i
\end{equation}
%\quad \quad \quad \quad \quad subject to
\begin{subnumcases}
{\label{constraint4causal_formualtion_prop}}
\beta_i E \subseteq  \alpha_i S_i, \quad \forall i\in \mathcal{N} \label{polytopecontain_causal_prop} \\
\sum_{i=1}^N \beta_i=1, \\
\alpha_i=1,  \quad \forall i\in \mathcal{N}\setminus \mathcal{N}_s,\\
\alpha_i\geq0,  \quad \forall i\in \mathcal{N}.
\end{subnumcases}
The optimal value of (\ref{causality4proportaional}) provides an upper bound on (\ref{resourceprocurement_causality}). Interestingly, the optimal solution to (\ref{causality4proportaional}) has the following properties:
\begin{itemize}
\item It maximizes the use of non-scalable resources. Scalable resources are procured only if non-scalable resources are not enough. 
\item When non-scalable resources are not enough, it only procures a single scalable resource. All remaining signals are allocated to this resource. 
\end{itemize}
To illustrate the first property, we define $\bar{\beta}_i$ as the maximum ratio  that can be assigned to the non-scalable resource $i$. Formally, for $i\in \mathcal{N}\setminus \mathcal{N}_s$,  $\bar{\beta}_i$ is defined as:
\begin{align}
\label{optimalsol4nonscale}
\bar{\beta}_i=&\arg \max_{\beta_i} \beta_i \\
&\begin{cases}
\beta_i E \subseteq S_i, \\ \nonumber
0\leq \beta_i\leq 1.  
\end{cases}
\end{align}
We argue that at the optimal solution to (\ref{causality4proportaional}), all non-scalable resources are fully utilized, i.e., $\beta_i=\bar{\beta}_i$ for $\forall i\in \mathcal{N}\setminus \mathcal{N}_s$. This is because  the amount of non-scalable resource is fixed and does not affect the cost of (\ref{causality4proportaional}).  If more signals are allocated to non-scalable resources, less is allocated to scalable resources. then less scalable  resources is needed, and the procurement cost is reduced.   Therefore, at the optimal solution, $\beta_i=\bar{\beta}_i$ for all $\forall i\in \mathcal{N}\setminus \mathcal{N}_s$. Formally, this can be summarized as the following proposition:
\begin{proposition}
\label{nonscalableresoruceoptiml}
Assume that $\sum_{i\in \mathcal{N}\setminus \mathcal{N}_s} \bar{\beta}_i<1$. If $(\alpha_1^*,\ldots,\alpha_N^*, \beta^*)$ is an optimal solution to (\ref{causality4proportaional}), then  $\beta_i^*=\bar{\beta}_i$ for $\forall i\in \mathcal{N}\setminus \mathcal{N}_s$, 
\end{proposition}
%\begin{proof}
%We prove this proposition by contradiction. Assume otherwise, i.e., there is some $j\in \mathcal{N}\setminus \mathcal{N}_s$ so that $\beta_j^*<\bar{\beta}_j$. Since $\sum_{i\in \mathcal{N}\setminus \mathcal{N}_s} \bar{\beta}_i<1$, there exists $k\in \mathcal{N}_s$ so that $\beta_k>0$. Now consider a new allocation policy that modifies $\beta^*$ by replacing $\beta_j^*$ with $\beta_j^*+\epsilon$ and replacing $\beta_k^*$ with $\beta_k^*-\epsilon$.  $\epsilon$ is such that $\beta_j^*+\epsilon\leq \bar{\beta}_j$ and $\beta_k^*-\epsilon\geq 0$. All other proportions remain the same. Since $\beta_k^*E \subseteq \alpha_k^* S_k$, we have $(\beta_k^*-\epsilon)E \subseteq \alpha_k^* \dfrac{\beta_k^*-\epsilon}{\beta_k^*} S_k$. This indicates that under the new allocation policy, buying $\alpha_k^*\dfrac{\beta_k^*-\epsilon}{\beta_k^*}$ units of resource $k$ is enough. Therefore, the new allocation policy leads to a strictly less procurement cost than $\beta^*$ does. A contradiction.   
%\end{proof}
The proof is simple, thus omitted. We comment that the assumption $\sum_{i\in \mathcal{N}\setminus \mathcal{N}_s} \bar{\beta}_i<1$ has no loss of generality. This is because if otherwise, the signals can be covered by the non-scalable resources, and no procurement is needed. 


The second property of the optimal solution to (\ref{causality4proportaional}) can be summarized as the following proposition:
\begin{proposition}
\label{meritorderproposition}
Assume that $\sum_{i\in \mathcal{N}\setminus \mathcal{N}_s} \bar{\beta}_i<1$, then there exists $j\in \mathcal{N}_s$ so that $(\alpha_1^*,\ldots,\alpha_N^*, \beta^*)$ is an optimal solution to (\ref{causality4proportaional}) and  $\alpha_i^*=0$ for $\forall i\neq j, i\in  \mathcal{N}_s$.  
\end{proposition}
\begin{proof}
For each $i\in \mathcal{N}_s$, define $k_i$ as the smallest $\alpha_i$ such that $E\subseteq \alpha_i S_i$. Assume that $k_i$ exits for all $i\in \mathcal{N}_s$. This assumption has no loss of generality,  since if $k_i$ does not exist for some $i$,  then there is no $\alpha_i$ such that $\beta_i E \subseteq \alpha_iS_i$ when $\beta>0$. In this case,   the optimal solution to (\ref{causality4proportaional}) has to  satisfy $\alpha_i=\beta_i=0$. This means the resource $i$ is neither used nor procured, so we can remove it from $\mathcal{N}_s$

Based on the definition of $k_i$, $E\subseteq \alpha_i S_i$ is  equivalent to $\alpha_i\geq k_i$, and the constraint (\ref{polytopecontain_causal_prop}) is equivalent to $\alpha_i\geq k_i\beta_i$. Plug this into (\ref{polytopecontain_causal_prop}). According to Proposition (\ref{nonscalableresoruceoptiml}), the resource procurement problem (\ref{causality4proportaional}) becomes:
\begin{align}
\label{intermproposition5}
&\min_{\alpha_1,\ldots,\alpha_N, \beta} \sum_{i\in \mathcal{N}_s} \alpha_i p_i  \\
&\begin{cases}
\alpha_i\geq k_i \beta_i, \quad \forall i\in \mathcal{N}_s  \\ \nonumber
\sum_{i\in \mathcal{N}_s} \beta_{i}=1 - \sum_{i\in \mathcal{N}\setminus \mathcal{N}_s} \bar{\beta}_i, \\ \nonumber
0\leq \beta_i \leq 1, \forall i\in \mathcal{N}_s. \nonumber 
\end{cases}
\end{align}
Clearly, at the optimal solution, we have $\alpha_i=k_i\beta_i$ for all $i\in \mathcal{N}_s$. Then  (\ref{intermproposition5}) is equivalent to:
\begin{align*}
&\min_{\{\beta_i, i\in \mathcal{N}_s\}} \sum_{i\in \mathcal{N}_s} k_i p_i \beta_i \\
&\begin{cases}
\sum_{i\in \mathcal{N}_s} \beta_{i}=1 - \sum_{i\in \mathcal{N}\setminus \mathcal{N}_s} \bar{\beta}_i,\\ \nonumber
0\leq \beta_{i}\leq 1, \quad \forall i\in \mathcal{N}_s.
\end{cases}
\end{align*}
Rank all resource in the ascending order of $k_ip_i$.  At the optimal solution,  only resources with the smallest $k_ip_i$ is selected. This competes the proof.
\end{proof}
Proposition \ref{meritorderproposition} indicates that under proportional allocation policy, each scalable resource has a ``virtual price" $k_ip_i$. It depends on the unit price $p_i$ and the shape of the polytope $S_i$. At the optimal solution, only the ``cheapest" resources are selected. This is similar to the merit order in electricity market. 

\begin{remark}
A natural extension of the proportional allocation policy is the time-varying proportional allocation policy. The time-varying policy also has a fixed proportion $\beta$, but $\beta$ can be different at different times. Under time-varying proportional allocation policy, Proposition \ref{meritorderproposition} no longer holds, but it provides a tighter upper bound on $J^{**}$ than (\ref{causality4proportaional}) does. 
\end{remark}





\subsubsection{Affine Causal Allocation Policy}
Next, consider a more general class of policies:
\begin{definition}
\label{linearpolicy}
The causal allocation policy $\gamma(\cdot)$ is affine if for any $i\in \mathcal{N}$ and $t\in \mathcal{T}$, there exists $C_i^t\in \mathbb{R}^t$ and $D_i^t\in \mathbb{R}$ such that:
\begin{align}
\label{affinepolicydef}
\begin{cases}
 \gamma_i^t(e^{1:t})=C_i^t [e^1,\ldots,e^t]^T+D_i^t, \\
 e^t=\sum_{i=1}^N \gamma_i^t(e^{1:t}), \quad \forall e\in E. 
\end{cases}
\end{align}
\end{definition}
The definition (\ref{affinepolicydef}) dictates that $\sum_{i=1}^N D_i^t=0$ for all $t\in \mathcal{T}$. 

\begin{remark}
 The size of $C_i^t$ increases with respect to $t$. Let $\bar{C}_i^t$ be a vector in $\mathbb{R}^T$ so that $\bar{C}_i^t=[C_i^t,0,\ldots,0]$. Define $C_i$ as a matrix in $\mathbb{R}^{T\times T}$ so that  $C_i=[\bar{C}_i^1,\ldots,\bar{C}_i^T]^T$. By definition, $C_i$ is a lower-triangular matrix. It is a causal policy: in each row $t$, the decision depends on the information up to time $t$, and entries after $t$ are $0$. When $C_i$ is a diagonal matrix, it corresponds to the time-varying proportion allocation policy. When $C_i$ is a diagonal matrix and its diagonal entries are identical, it represents proportional allocation policy.  Therefore, both proportional   and time-varying proportional allocation policies are special cases of the affine causal policy.      
\end{remark}

Under affine causal policy, the resource procurement problem (\ref{resourceprocurement_causality}) can be transformed  to a linear program:
\begin{theorem}
\label{linearupperbound}
Assume that $\gamma(\cdot)$  satisfies (\ref{affinepolicydef}), then the resource procurement problem (\ref{resourceprocurement_causality}) is equivalent to the following linear program:
\begin{equation}
\label{resourceprocurement_causal_linear}
\hspace{-4.5cm} \min \sum_{i=1}^{N} \alpha_i p_i
\end{equation}
\begin{subnumcases}{\label{constraint4causal}}
v_m^t=\sum_{i=1}^N C_i^t[v_m^1,\ldots,v_m^t]^T, \quad \forall m\in \mathcal{M},t\in \mathcal{T} \label{conservationofall_linear}\\
A_i[\gamma_i^1(v_m^1),\ldots,\gamma_i^T(v_m^{1:T})]^T\leq \alpha_iB_i,  \quad \forall i,m, \label{feasibleset_i}\\
\alpha_i=1, \quad \forall i\in \mathcal{N}\setminus \mathcal{N}_s, \\
\alpha_i\geq 0,  \quad \forall i\in \mathcal{N},
\end{subnumcases}
The decision variables are $\alpha_1, \ldots, \alpha_N$ and $C_i^t$ for $\forall i,t$.
\end{theorem}
\begin{proof}
Since the allocation policy is affine, the resource procurement problem can be written as follows:
\begin{equation}
\label{resourceprocurement_causal_linear_intermediate}
\hspace{-4.5cm} \min \sum_{i=1}^{N} \alpha_i p_i
\end{equation}
%\quad \quad \quad \quad \quad subject to: 
\begin{subnumcases}{\label{constraint4causal_intermediate}}
e^t=\sum_{i=1}^N C_i^t[e^1,\ldots,e^t]^T, \quad \forall j\in \mathcal{M},t\in \mathcal{T}, \label{conservationofall_linear_1}\\
A_i[\gamma_i^1(e^1),\ldots,\gamma_i^T(e^{1:T})]^T\leq \alpha_iB_i, \forall i\in \mathcal{N}, \\
\alpha_i=1, \quad \forall i\in \mathcal{N}\setminus \mathcal{N}_s, \\
\alpha_i\geq 0,  \quad \forall i\in \mathcal{N}, \label{feasibleset_i_1}\\
\forall e\in E. \label{robustconstrinat}
\end{subnumcases}
where $\gamma_i^t(\cdot)$ satisfies (\ref{affinepolicydef}). 
Note that constraints (\ref{conservationofall_linear_1})-(\ref{feasibleset_i_1}) is linear with respect to $e$. Therefore, (\ref{conservationofall_linear_1})-(\ref{feasibleset_i_1}) holds for all $e\in E$ if and only if it holds for all vertices of $E$. This is exactly  (\ref{constraint4causal}).
\end{proof} 
 
Based on Theorem \ref{linearupperbound}, the solution to (\ref{resourceprocurement_causal_linear}) is the optimal linear causal policy. The optimal value of (\ref{resourceprocurement_causal_linear}) provides an upper bound on $J^{**}$.



\begin{figure}[t]%
\centering
\includegraphics[width = 0.5\linewidth]{figureshringking}
\caption{The variation of the random signal is small,   $E$ is a long stick around the axis $e^1=e^2$. Here $T=2$.}
\label{figureshringking}
\end{figure}

\begin{remark}
In many problems of interest, the variation of the signal is small relative to the range of possible values of $e^1$. This can be exploited to bound the price of causality. For example, in the reserve procurement problem, the operator predicts in one-day ahead that the imbalance signal at the first 5-minute could range from $-10MW$ to $10MW$, i.e., $-10\leq e^1 \leq 10$. With high probability,  $e_t-e_1$ could range from $-1MW$ to $1MW$ for all $t$ within the first hour. In this case, $E$ is a long stick around  the line $e^1=\cdots=e^T$. An example of this case is shown in  Figure \ref{figureshringking}, where $T=2$. Since the variation is small, the random signals in the future are almost known after $e^1$ is revealed. Therefore, we expect the price of causality to be small.  
\end{remark}




























